Duality between Coronavirus Transmission and Air-based Macroscopic Molecular Communication

This contribution exploits the duality between a viral infection process and macroscopic air-based molecular communication. Airborne aerosol and droplet transmission through human respiratory processes is modeled as an instance of a multiuser molecular communication scenario employing respiratory-event-driven molecular variable-concentration shift keying. Modeling is aided by experiments that are motivated by a macroscopic air-based molecular communication testbed. In artificially induced coughs, a saturated aqueous solution containing a fluorescent dye mixed with saliva is released by an adult test person. The emitted particles are made visible by means of optical detection exploiting the fluorescent dye. The number of particles recorded is significantly higher in test series without mouth and nose protection than in those with a wellfitting medical mask. A simulation tool for macroscopic molecular communication processes is extended and used for estimating the transmission of infectious aerosols in different environments. Towards this goal, parameters obtained through self experiments are taken. The work is inspired by the recent outbreak of the coronavirus pandemic.

==> Commentary.tex <==
\section*{Letter to the Editor}

{\color{blue}The authors would like to thank the reviewers for their valuable feedback. All suggestions and recommendations have been taken into account. Thanks to the given advise, the paper has greatly improved. }



\textbf{Reviewer: 1}

I would highly recommend that the authors make the experimental data associated with this work publicly available, e.g., via dataport or some similar repository. The dataset could then be cited by the manuscript and be readily accessible to the wider community.

\begin{quote}
\color{blue} We will publish video files and photographs of our experiments via IEEE DataPort once the manuscript is accepted for publication. 
\end{quote}

- the modeling assumptions for molecule release seem reasonable but are also not supported with references. Where does the breathing rate come from? Is it common to model speaking as a 2-state Markov process? Have other models generated sneeze or cough events as Bernouilli trials? Are these all developed from the authors' own intuition? They don't seem like necessarily novel ideas, so clarification is needed.

\begin{quote}
\color{blue}Many thanks for this comment. We revised the text as follows:

\subsubsection{Breathing}
The continuous breathing of a human is influenced by the physical load on the body. The breathing pattern at rest of 12-16 breaths per minute~\cite{Barrett2010} can increase with higher physical activities, resulting in a higher aerosol emission rate and also larger emission volumes following deeper breaths. 

\subsubsection{Speaking}
Human speaking can be modeled as a two-state Markov process~\cite{Jaffe1964}. The states represent the talking and silence periods. This discrete-time model is characterized by the transition probabilities between the states and the retention probabilities for staying in the current state. This represents the fact that a human, currently being in speaking state, might eventually stay in this state for the next time step with a higher probability than switching into the silent state. Whenever a human is speaking, an average aerosol distribution is emitted into the environment. This simplification takes into account differences in languages and phonetic characteristics, as the transition probabilities may be time-varying.

\subsubsection{Coughing and Sneezing}
Coughing and sneezing as randomly and sparsely occurring events can be modeled for each time step in terms of a Bernoulli trial, where the user might eventually emit aerosols in terms of a cough or sneeze, or stay in normal breathing state. The parameter for the resulting Poisson process is influenced by the infection state of the user. The intensity increases for an infected human, which resembles a higher probability for coughing and sneezing, whereas a healthy human might cough or sneeze very rarely. This concept has been introduced in~\cite{Penrose1996}.
\end{quote}

- how did the authors arrive at the "natural" equation for estimating the maximum travel distance? Besides the units working out, this formulation does not seem intuitive. Was the "2" coefficient a fitted parameter or arbitrarily chosen?

\begin{quote}
\color{blue} This is a very good point. The equation describes the maximum flight distance of an object thrown with velocity $v$ perpendicular to the ground from height $h_0$ given the gravitational acceleration $g$. The equation is derived from the time an object falls from height $h_0$ to the ground: $t=\sqrt{2h_0 / g}$. Inserting this result into the flight distance (e.g., the horizontal part of the equation of motion) results in $d = v_0 \, t = v_0 \, \sqrt{2h_0 / g}$.
\end{quote}

- what method of analysis was used to arrive at the droplet diameter and distance distributions? Were the photographs analyzed manually or was there an automated approach?

\begin{quote}
\color{blue}
Many thanks for this comment. The text has been extended as follows:

``To estimate the droplet diameter distribution shown in Fig.~\ref{fig:aerosol_diameter_distribution}, the photographs are analyzed with an automated approach employing Matlab.
A tape measure laid out on the floor enables a calculation of the size of the droplets on the floor given the recorded pixels.
A calibration measurement obtained by an industrial sprayer with a defined droplet radius of $\SI{3.3}{\micro\meter}$ is then used to relate the radius of circles on the floor to the actual droplet sizes in the air. 
This processing is accompanied by an analysis of distance measurements, as shown in Fig.~\ref{fig:aerosol_distance_distribution}.''

\end{quote}

- It is noted that 1-100 microns is the diameter range of interest; were 1 micron droplets reliabily measured with the techniques used? This would seem to be very difficult to do from photographs

\begin{quote}
\color{blue} This question has been addressed in a calibration step as explained in the previous comment.
\end{quote}

- even though no fluorescence was observed in the case with the test subject wearing a mask, it would be useful to present visual evidence of this as a control/comparative case.

\begin{quote}
\color{blue} We have added to the paper that the mask under investigation additionally fulfills Type IIR EN 14683:2019, having a bacterial filtration efficiency of more than 98~\% and an aerosol filtration percentage of 80~\% minimum. 
This suggests that visual evidence can hardly be expected.  The latter fact is added in the conclusions. As mentioned in the first answer, supporting material will be published upon acceptance. 
\end{quote}

- more information about the simulator would be useful, especially given that the only reference for it is the conference paper [30] and it is noted that the implementation in this work is an extension of that implementation. Is there a reference for the initial implementation before extension to macroscopic MC? Furthermore, how can readers access the software?

\begin{quote}
%\color{gray} TODO - Berlin: replaced reference, more description, link to source

\color{lukas} This is indeed a very important aspect. We replaced the reference with a more up-to-date publication~\cite{drees2020efficient} which had not yet been published at the time of our previous submission.
Furthermore, we added a link to the simulator web page, where references to the source code and documentation can be found.
\end{quote}

- the abstract does not summarize the results. What does the modeling enable?

\begin{quote}
\color{blue} We thank the reviewer for this suggestion. The abstract has been extended as follows:

``Modeling is aided by experiments that are motivated by a macroscopic air-based molecular communication testbed.
In artificially induced coughs, a saturated aqueous solution containing a fluorescent dye mixed with saliva is released by an adult test person. 
The emitted particles are made visible by means of optical detection exploiting the fluorescent dye. 
The number of particles recorded is significantly higher in test series without mouth and nose protection than in those with a well-fitting medical mask.
A simulation tool for macroscopic molecular communication processes is extended and used for estimating the transmission of infectious aerosols in different environments. 
Towards this goal, parameters obtained through self experiments are taken.'' 
\end{quote}

- for fig. 1, it is unclear why the arrows are not all connected to the droplet

\begin{quote}
\color{blue}Following this recommendation, we revised the text as follows: 

``Fig. 1: Forces acting on aerosols in an air-based environment: bouyancy force $F_\text{B}$ and air drag force $F_\text{D}$ act mainly on the air-stream that is expelled from the mouth or nose, whereas advection force $F_\text{A}$ and gravitational force $F_\text{G}$ act on the aerosols themselves.
The temperature gradient is given through the minimum temperature $T_\text{min}$ of the air in the environment and the maximum temperature $T_\text{max}$ of the liquid in the oral cavity.''
\end{quote}

- fig. 2 labelling does not make it clear which users are healthy vs infectious. Presumably the red pathway is the infectious one, but at best this is inferred

\begin{quote}
\color{blue}Again, we thank the reviewer for the suggestion. The text has been revised:

``Fig. 2: Sketch of a multiuser scenario with one infected transmitter (red) emitting infectious aerosols into an air-based environment with three healthy receivers (blue) at a time instance $t$. The lines show possible trajectories.''
\end{quote}

- perhaps it is generally accepted in virology that an infected person will have both infectious and non-infectious particles released at the same time. To me this does seem somewhat intuitive, but nevertheless I think it would be best to have a citation to support this modeling detail

\begin{quote}
\color{blue}Giving evidence here is indeed important. The text has been revised as follows: 

``The probability that a droplet contains viruses is closely related to its initial volume~\cite{Stadnytskyi2020}.''
\end{quote}

- is there a need to include the case where a person is sneezing or coughing frequently but is not infectious with the pathogen being considered? This seems like a reasonable "false positive" scenario

\begin{quote}
\color{blue} We thank the reviewer for this comment. The revised version of the manuscript mentions the case of non-infectious particles as well. 
\end{quote}

- is there a reference for Schlieren imaging?

\begin{quote}
\color{blue}We added a reference and revised the text as follows:

``The advantage of fluorescent particles becomes apparent, as they stay visible under longwave ultra-violet (UVA) light even after settlement. Commonly used techniques like shadowgraph~\cite{Tang2012} or Schlieren imaging~\cite{Tang2009} do not provide this feature.''
\end{quote}

- how long did it take to heat the Uranine solution in the mouth? How was it confirmed that it was heated to body temperature?

\begin{quote}
\color{blue} We added more details on the experiment as follows:

``The tests are carried out with a test person to obtain sufficient parameters for the simulation environment: About $\SI{10}{\milli\liter}$ of a saturated aqueous solution containing the fluorescent dye Uranine (mixing ratio: $\SI{1.54}{\gram\per\liter}$) is taken in through the mouth and mixed with saliva. Over a period of two minutes the liquid in the mouth cavity is heated to body temperature.''\\

The initial temperature of the water has been about 20$^{\circ}$C, which is the ambient temperature reported in the manuscript. The temperature inside the mouth has been about 36$^{\circ}$C.  To heat-up one gram of water by one degree, one calorie is required.  Consequently, about 160 calories were needed. Towards this goal, the test person gargled intensely over a period of two minutes in order to reach the desired temperature gradient.  By means of a thermal imaging camera PeakTech 5605, we have verified the success.    
\end{quote}

- what was the approximate cough frequency within an interval, how long after each cough was the floor photographed, and was the room known to be "clear" of particles before the start of a new cough interval?

\begin{quote}
\color{blue}We see that we have been too brief here. We added more details on the experiment as follows:

``Four test series were carried out without a protective mask and one test series with a mask. Each test series consists of five consecutive, artificially triggered coughs, each about 15 seconds apart. The floor was photographed before each new cough and after the final cough. Between the test series, a new portion of Uranine solution was taken into the mouth and warmed to body temperature, and the floor was cleaned of the residues of the previous test series.''
\end{quote}

- there are occasional areas where the use of definite articles seems inappropriate, e.g., "leading to the infection of the humans" (p.2)

\begin{quote}
\color{blue}We thank the reviewer for this advice.  The paper has been revised with regard to the note.
\end{quote}

- is "viral load in collected samples of particles" really a "field"?

\begin{quote}
\color{blue}The text was indeed a bit misleading. We revised it as follows:

``Further research was conducted to determine the viral load in collected samples of particles from surfaces~\cite{Pan2020,Rothe2020,To2020}, as well as the influence of varying activity loads on the human body by the emitted viral load~\cite{Buonanno2020}.''
\end{quote}

- cell-to-cell communication would seem to me to be multicellular and not "unicellular", as claimed

\begin{quote}
\color{blue}We thank the reviewer for pointing this out. We updated the text to be more precise:

``From an evolutionary perspective, this concept has proven to be effective
and can be observed in the communication of unicellular organisms via molecules in fluid environments~\cite{Bassler2002},
or in macroscopic communication through pheromones in the air~\cite{Bassler2006}.''
\end{quote}

- "MC is believed to improve a wide range of applications" - this wording seems unclear about has been done vs what may be possible. The papers cited refer primarily to as-yet undeveloped technologies; what is MC currently improving, as suggested?

\begin{quote}
\color{blue}Following this advise, we improved the text as follows:

``Starting from the microscopic domain with application areas inside the human body like targeted drug delivery~\cite{Akyildiz2010}, improved diagnosis and treatment with lab-on-a-chip devices to accelerate and refine the medical procedure~\cite{Nakano2013,Akyildiz2019}, in the domain of bio-sensors and intelligent materials~\cite{Nakano2005}, and even beyond in-body applications~\cite{dressler2015connecting}, MC is believed to improve a wide range of applications. 
In addition to the theoretical discussions of MC application areas, there is currently a lack of practical implementations, as this requires a high degree of cooperation between engineers from different disciplines~\cite{Jamali2016}. The macroscopic domain of MC mainly focuses on industrial and smart city applications for instance, where traditional radio communication might be challenging to accomplish. In order to understand the underlying principles and the overall system better, several testbeds have been developed~\cite{Jamali2019} based for example on magnetic nanoparticles~\cite{Unterweger2018}, alcohol molecules~\cite{Farsad2013}, or fluorescent dyes~\cite{Atthanayake2018, Bhattacharjee2020a, Bhattacharjee2020b} using a fluid-based or air-based environment.''
\end{quote}

- "differently sized particles" - "different-sized particles". Or if "differently" was also intended to apply to velocity and direction, then "different particles sizes, initial velocities, and emission directions"

\begin{quote}
\color{blue}We updated the grammar here as follows:

``These include the amount of particles released with a certain probability distribution of different particle sizes, initial velocities, as well as emission directions.''
\end{quote}

- "maximize the likelihood decision rule" - how does one maximize a rule? Should this be "maximize the decision likelihood"?

\begin{quote}
\color{blue}The wording was indeed not correct. The text has been revised as follows:

``A detection problem to maximize the decision likelihood is formulated and the corresponding missed detection probability is minimized.''
\end{quote}

- The sentence introducing [35] starts with "Even more recently ..." but this is confusing as [35] is cited in the previous sentence

\begin{quote}
\color{blue}We updated the text following this advise:

``In \cite{Khalid2019}, a biosensor is assumed at the receiver side. The focus is on outdoor environments. In the follow-up work \cite{Khalid2020}, a complete system model is presented and an end-to-end mathematical model is derived for the transmission channel under certain constraints and boundary conditions. Additionally, the system response for both continuous sources such as breathing and jet or impulsive sources such as coughing and sneezing is studied. In addition to transmitter and channel, a receiver architecture composed of air sampler and silicon nanowire field-effect transistor is assumed. A detection problem to {\color{blue}maximize the decision likelihood} is formulated and the corresponding missed detection probability is minimized. Several numerical results are presented to observe the impact of parameters that affect the performance and justify the feasibility of the proposed setup in related applications.

Even more recently and independent of the presented work, the biosensor-based detector is replaced by an absorbing detector in the form of a healthy human located at a certain distance from the emitter~\cite{Gulec2020}. That way, the spreading mechanism of infectious diseases by airborne pathogen transmission between two humans could be modeled for the first time using the principles of MC. If a certain amount of aerosols is able to reach the receiver's detection space, the receiver is expected to be infected. This corresponds to a successful transmission of information between the transmitter and the receiver via a distorted channel in traditional MC. An end-to-end system model is proposed with emphasis on the indoor environment, predicting the infection state of a human. The corresponding infection probability is derived. 

Contrary to the classical data transmission approach, epidemiologists aim to reduce the number of successful transmissions.
In other words, in data transmission, a maximization of the mutual information is targeted, whereas in the case of virus transmission, a minimization of the mutual information is targeted. Based on the modeling assumptions, rules concerning ``social distancing'' are suggested. In the state-of-the-art \cite{Khalid2019,Khalid2020,Gulec2020}, the MC concept has been restricted to peer-to-peer links.''
\end{quote}

- The sentence "Based on the modeling assumptions, rules concerning 'social distancing' are suggested" comes after the current paragraph appears to proceed from summarizing [35] to contrasting the goals in data vs virus transmission. Thus, it is not entirely clear that the authors are still discussing [35]

\begin{quote}
\color{blue}Please see the previous comment on how we dealt with the recommendation.
\end{quote}

- "fluorescence dye" - "fluorescent dye"

\begin{quote}
\color{blue}The text has been revised:

``Channel modeling is aided by air-based experiments using a fluorescent dye in conjunction with optical detection~\cite{Bhattacharjee2020a}.''
\end{quote}

- would it make more sense to "translate" the comm scheme to virology instead of "transfer"?

\begin{quote}
\color{blue}Translation is indeed the better wording here. We revised the text as follows:

``This scenario resembles an elementary peer-to-peer communication scheme with two users. To enable the translation to the field of virology, the scenario must be extended to several users who can both send and receive aerosols in a three dimensional (3D) environment.''
\end{quote}

\textbf{Reviewer: 2}

The paper introduces a communication theoretical approach to the airborne aerosol and droplet transmission by employing both the experimental and simulation results. In my opinion, the paper is very well-written and the contribution provided by the paper deserves to be published in order to disseminate the given important insights in overcoming the severe pandemic. 

\begin{quote}
\color{blue} We thank the reviewer for these very encouraging remarks.
\end{quote}

Before a possible publication process, it would be great to further clarify how the results of the experiments and simulations can be interpreted in terms of conventional performance metrics in the communication theory and networking.

\begin{quote}
\color{revised}
Many thanks for this comment.  There are indeed many analogies between the two areas.  
A new Section~\ref{sec:relations} entitled ``Relation to Communication Theory and Networking'' has been added:

\begin{table}[ht]
\caption*{\color{revised}TABLE III: Relationship between conventional performance metrics and infectious particle transmission.}
\centering
\color{revised}
\begin{tabularx}{\linewidth}{XX}
\toprule
Traditional performance metric & Infectious particle transmission \\
\midrule
Received power (signal-to-noise ratio)  & Heat map \\
Communication range                     & Infection range \\
Beamforming                             & Shapes of aerosol clouds \\
Signal blocking / shadowing             & Masks, protective screens, and other obstacles \\
Retransmission                          & Consecutive respiratory events \\
\midrule
Outage, bit/frame error rate            & Probability of infection \\
Connectivity                            & Chain of infection, reproduction number \\
Throughput, data rate                   & Viral load \\
Latency (jitter)                        & Incubation time \\
Number of communication channels        & Number of contacts \\
\bottomrule
\end{tabularx}
\end{table}

``The duality elaborated in Section~\ref{sec:scenario} makes it possible to relate selected results and conclusions of the experiments and simulations to traditional performance metrics in communication theory and networking: 
%
\begin{enumerate}
    \item The spatially distributed received power (or the signal-to-noise ratio, respectively) relates to the heat map in Fig.~\ref{fig:simulation_heatmap}.
    \item The communication range corresponds to the range of infection. 
    The distribution of droplet flight distances is depicted in Fig.~\ref{fig:aerosol_distance_distribution}. The maximum range, $d_\mathrm{max}$, has been confirmed analytically.
    \item The shapes of the emitted aerosol clouds depend on the type of respiratory event and are analogous to beamforming, i.e., to directional transmission of information. 
    These shapes are considered in the simulation tool. 
    \item Signal blocking/shadowing is linked to masks, protective screens, and other obstacles.
    \item Retransmission is related to consecutive respiratory events. 
\end{enumerate}

These and additional performance metrics that are not further evaluated in this contribution (such as probability of infection, chain of infection, viral load, incubation time) are depicted in Table~\ref{table:relation}.''
\end{quote}

\textbf{Reviewer: 3}

1- Page 1, the right column, line 16: Please provide reference(s) for stating the size of aerosols. You can use for example [38] for referring to. 

\begin{quote}
\color{blue}We thank the reviewer for this helpful comment. The text has been revised  as follows:

``The literature uses the term ``aerosol'' for a wide range of particles, starting with aerosols of a few hundred nanometers in diameter up to droplets with a diameter of about $\SI{100}{\micro\meter}$~\cite{Hinds1999}.''
\end{quote}

2- In Section I (Introduction), the novelty of your work is highlighted with the experimental data and modeling of transmitters from the MC point of view. However, as you mentioned in the literature review, these novelties have been done in your previous works, [30] and [36], and also the difference between your work and [32] and [33] is not visible for the reader. I strongly suggest highlighting your work’s contributions and also, the differences between your work and the previous similar works in the revised version of the manuscript.

\begin{quote}
\color{blue} 
In the manuscript, it is mentioned that the state-of-the-art [32], [33] (now: \cite{Khalid2019}, \cite{Khalid2020}) considers
\begin{itemize}
    \item peer-to-peer links,
    \item outdoor environments, and  
    \item bio sensors as receivers.
\end{itemize}
In contrast to that our contribution takes into account multiuser scenarios, indoor environments, and human receivers. Respiratory events like breathing, speaking, coughing, or sneezing are modeled by respiratory-event-driven molecular concentration shift keying, as motivated by [36] (now: \cite{Bhattacharjee2019}). Additionally, own experiments where conducted and a simulation tool has been extended. In [30] (now: \cite{Bhattacharjee2020b}) a pipe-based testbed is proposed as a measurement environment. In contrast to that the new experiments where conducted in a quasi-unbounded environment. The manuscript has been extended accordingly.
\end{quote}

3- On Page 1, left column, line 43, you have stated that “the transmission of infectious aerosols with coronavirus RNA is modeled by a multiuser MC scenario”. However, I did not find any explanation and/or biological modeling regarding RNA roles in changing the cells’ functionalities.

\begin{quote}
\color{blue} This is a very good point. The text has been revised as follows:

``Airborne aerosols are able to carry pathogens, for example in the form of viral ribonucleic acid (RNA), that might infect other humans when inhaled into the respiratory tract~\cite{Bourouiba2014,Cann2005}.''
\end{quote}

4- Please provide reference(s) for stating the shrinkage of droplets diameter on Page 2, column left, line 47.

\begin{quote}
\color{blue}We added a reference here as follows:

``Following the same temperature profile as the expelled air stream, the aerosols are subject to an evaporation process resulting in the shrinkage of the droplet diameter~\cite{Ranz1952}.''
\end{quote}

5- In Section II (Principles of Aerosol Transport), you studied the ways that aerosols can propagate in the environment. There is also the possibility of breaking up a larger droplet into smaller droplets. I suggest the authors also cover this possibility in their work. [R1] can maybe helpful.
[R1]: doi:10.1001/jama.2020.4756

\begin{quote}
\color{blue} We added this reference as suggested:

``Larger and heavier droplets are either fragmented into smaller droplets~\cite{Bourouiba2020} or quickly forced to the ground.''
\end{quote}

6- I am not sure that the movements of the transmitters are random in the paper. Because the lines in Fig. 2 are predetermined, thus meaning that they are moving deterministically, not randomly. Please explicitly state the movements’ mechanism in the paper. It is also worth noting the transmitters’ movements mechanism in the abstract.

\begin{quote}
\color{blue}This is indeed correct. We updated the text as follows:

``Fig. 2: Sketch of a multiuser scenario with one infected transmitter (red) emitting infectious aerosols into an air-based environment with three healthy receivers (blue) at a time instance $t$. The lines show possible trajectories.''
\end{quote}

7- I suggest bringing your experimental report about the preventing effects of FFP1 medical mask in the abstract. It is an important and beneficial conclusion in the molecular communication society.

\begin{quote}
\color{blue} We thank the reviewer for this suggestion. This is in line with comments by Reviewer~1. The abstract has been extended accordingly (see above). 
\end{quote}

8- I did not find the simulation of the multi-user scenario introduced in Section III (Scenario Under Investigation) in Section IV (Measurement Results). I suggest providing the simulation of your statement of the multi-user scenario. 

\begin{quote}
\color{blue} This is a good point.  Section IV actually covers experimental results as well as simulation results.  In the experimental results focus has indeed been on a single-user scenario, because we believe that in good approximation particle clouds emitted by several people will superimpose.  Regarding the Pogona simulation tool, the same setup has been chosen in order to verify the experiments. Of course, the simulation tool is more powerful in the sense that multiuser scenarios could be emulated as well, see https://www2.tkn.tu-berlin.de/software/pogona/ for source code and documentation. 

%This is indeed correct. We assume a multi-user scenario to be a superposition of multiple peer-to-peer communication links. We updated the text as follows:

%``This scenario resembles an elementary peer-to-peer communication scheme with two users. To enable the translation to the field of virology, the scenario must be extended to several users who can both send and receive aerosols in a three dimensional (3D) environment. A randomly selected proportion of users are assumed to be infected, emitting infectious particles during their respiratory events. This extended macroscopic MC scenario is shown in Fig.~\ref{fig:scenario_sketch}. All transceivers in the scenario are mobile. This results in a dynamic situation, where the distances between the users are varying.

%As the multiuser scenario is basically a superposition of multiple peer-to-peer communication links, therefore this paper presents the basic case of two transceivers with one infected and one uninfected user.''
\end{quote}

9- The authors also modeled the aerosol emission events in Section III but I did not find any simulation, experimental, or theoretical modeling through the paper. 

\begin{quote}
\color{blue}
% \todoTo{Berlin}{masc: I don't see what to respond to this comment as we modeled the aerosol emission through a coughing event.}

% \color{red} Vielleicht sollten wir verstärkt darauf hinweisen, dass eigene experimentelle Ergebnisse in den Pogona Simulator geflossen sind. 

We thank the reviewer for this useful advice and have expanded the description of our experimental concept:

``The industrial sprayer used as a transmitter in [33] is replaced by a test person emulating an infected  person.  As an example of the above mentioned respiratory events, successive coughs are induced. Key parameters obtained from the experiments like particle diameters and distance profile are used in the simulation tool.''
\end{quote}

10- I suggest the authors simulating the proposed emission events like speaking, breathing, sneezing, and coughing by the extended Pogona simulator and providing another figure. I strongly believe that it can greatly improve the paper.

\begin{quote}
\color{blue}
We thank the reviewer for this suggestion.
We plan to take this suggestion into account in our future efforts.

% Discussion on Slack, 2020-11-30:
% 
% Lukas Stratmann  15:07
% Gute Idee, das vor Weihnachten fertig zu bringen!
% Der Wunsch von Reviewer 1 deckt sich mit meinem Vorhaben, möglichst bald den Source Code zu veröffentlichen.
% Reviewer 3 schlägt ja auch die Simulation anderer emission events vor. Würde das nicht neue "Labor"-Experimente und Fotos voraussetzen?
% 
% Max Schurwanz  15:12
% Ja an sich schon, außer er erwartet so eine Abbildung, wo man sieht, dass die Partikel mit anderem Öffnungswinkel und anderen Geschwindigkeiten ausgestoßen werden.. Aber ich denke auch, dass wir darauf verzichten können und reinschreiben, dass das für zukünftige Veröffentlichungen ein sinnvoller Hinweis ist und berücksichtigt werden wird.
\end{quote}

11- I suggest that the authors summarize the modelings, novelties, and the main contributions of the paper in the conclusion section.

\begin{quote}
\color{blue} We are very grateful for the suggestion and have expanded the conclusions accordingly: 

``This paper exploits the duality between a viral infection process and macroscopic air-based molecular communication.  
It connects an engineering perspective with the medical domain of virus-laden airborne particles as disease spreading mechanism.
Novel contributions include the following aspects:
\begin{itemize}
    \item The transmission of infectious and non-infectious aerosols and droplets from human airways expelled through respiratory events is interpreted as a multiuser MC scenario. Infection chains are the root of reproduction. 
    \item Respiratory events like breathing, speaking, coughing, or sneezing are modeled by respiratory-event-driven molecular concentration shift keying. 
    \item Channel modeling is aided by human experiments employing a fluorescent dye.  The efficacy of a medical mask is verified.
    \item  The advanced MC Pogona simulation tool is extended to emulate aerosol transmission in different environments.
    Parameters feeding this tool are partly obtained by own experimental results.
\end{itemize}
The contribution paves the way to new opportunities and tools for analysis and prevention of infectious diseases caused by airborne pathogen transmission.\\

An optical particle detection technique previously employed in the area of air-based macroscopic MC is used as a basis to model the different respiratory events. Video recordings and existing knowledge about channel modeling from MC are combined to make more accurate predictions about the dispersion of aerosols in the ambient air using an advanced simulation environment. Possibly infectious particles are made visible using a fluorescent dye.''
\end{quote}

